Unified Multimodal Punctuation Restoration Framework for Mixed-Modality Corpus

The punctuation restoration task aims to correctly punctuate the output transcriptions of automatic speech recognition systems. Previous punctuation models, either using text only or demanding the corresponding audio, tend to be constrained by real scenes, where unpunctuated sentences are a mixture of those with and without audio. This paper proposes a unified multimodal punctuation restoration framework, named UniPunc, to punctuate the mixed sentences with a single model. UniPunc jointly represents audio and non-audio samples in a shared latent space, based on which the model learns a hybrid representation and punctuates both kinds of samples. We validate the effectiveness of the UniPunc on real-world datasets, which outperforms various strong baselines (e.g. BERT, MuSe) by at least 0.8 overall F1 scores, making a new state-of-the-art. Extensive experiments show that UniPunc's design is a pervasive solution: by grafting onto previous models, UniPunc enables them to punctuate on the mixed corpus. Our code is available at github.com/Yaoming95/UniPunc

==> ref_bak.tex <==

@inproceedings{christensen2001punctuation,
  title={Punctuation Annotation using Statistical Prosody Models},
  author={Christensen, Heidi and Gotoh, Yoshihiko and Renals, Steve},
  booktitle={ISCA Tutorial and Research Workshop (ITRW) on Prosody in Speech Recognition and Understanding},
  year={2001}
}

@inproceedings{kim2019deep,
  title={Deep recurrent neural networks with layer-wise multi-head attentions for punctuation restoration},
  author={Kim, Seokhwan},
  booktitle={ICASSP 2019-2019 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)},
  pages={7280--7284},
  year={2019},
  organization={IEEE}
}

@inproceedings{DBLP:conf/interspeech/SunkaraRBBK20,
  author    = {Monica Sunkara and
               Srikanth Ronanki and
               Dhanush Bekal and
               Sravan Bodapati and
               Katrin Kirchhoff},
  editor    = {Helen Meng and
               Bo Xu and
               Thomas Fang Zheng},
  title     = {Multimodal Semi-Supervised Learning Framework for Punctuation Prediction
               in Conversational Speech},
  booktitle = {Interspeech 2020, 21st Annual Conference of the International Speech
               Communication Association, Virtual Event, Shanghai, China, 25-29 October
               2020},
  pages     = {4911--4915},
  publisher = {{ISCA}},
  year      = {2020},
  url       = {https://doi.org/10.21437/Interspeech.2020-3074},
  doi       = {10.21437/Interspeech.2020-3074},
}

@inproceedings{DBLP:conf/icassp/YiT19,
  author    = {Jiangyan Yi and
               Jianhua Tao},
  title     = {Self-attention Based Model for Punctuation Prediction Using Word and
               Speech Embeddings},
  booktitle = {{IEEE} International Conference on Acoustics, Speech and Signal Processing,
               {ICASSP} 2019, Brighton, United Kingdom, May 12-17, 2019},
  pages     = {7270--7274},
  publisher = {{IEEE}},
  year      = {2019},
  url       = {https://doi.org/10.1109/ICASSP.2019.8682260},
  doi       = {10.1109/ICASSP.2019.8682260},
}

@inproceedings{klejch2017sequence,
  title={Sequence-to-sequence models for punctuated transcription combining lexical and acoustic features},
  author={Klejch, Ond{\v{r}}ej and Bell, Peter and Renals, Steve},
  booktitle={2017 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)},
  pages={5700--5704},
  year={2017},
  organization={IEEE}
}

@inproceedings{DBLP:conf/interspeech/BatistaCMT07,
  author    = {Fernando Batista and
               Diamantino Caseiro and
               Nuno J. Mamede and
               Isabel Trancoso},
  title     = {Recovering punctuation marks for automatic speech recognition},
  booktitle = {{INTERSPEECH} 2007, 8th Annual Conference of the International Speech
               Communication Association, Antwerp, Belgium, August 27-31, 2007},
  pages     = {2153--2156},
  publisher = {{ISCA}},
  year      = {2007},
}
a service of  Schloss Dagstuhl - Leibniz Center for Informatics	homebrowsesearchabout



@inproceedings{tilk2015lstm,
  title={LSTM for punctuation restoration in speech transcripts},
  author={Tilk, Ottokar and Alum{\"a}e, Tanel},
  booktitle={Sixteenth annual conference of the international speech communication association},
  year={2015}
}

@inproceedings{silva2021multimodal,
  title={Multimodal Punctuation Prediction with Contextual Dropout},
  author={Silva, Andrew and Theobald, Barry-John and Apostoloff, Nicholas},
  booktitle={ICASSP 2021-2021 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)},
  pages={3980--3984},
  year={2021},
  organization={IEEE}
}

@inproceedings{yi2020focal,
  title={Focal Loss for Punctuation Prediction.},
  author={Yi, Jiangyan and Tao, Jianhua and Tian, Zhengkun and Bai, Ye and Fan, Cunhang},
  booktitle={INTERSPEECH},
  pages={721--725},
  year={2020}
}


@inproceedings{pardede2019generalized,
  title={Generalized Filter-bank Features for Robust Speech Recognition Against Reverberation},
  author={Pardede, Hilman F and Zilvan, Vicky and Krisnandi, Dikdik and Heryana, Ana and Kusumo, R Budiarianto S},
  booktitle={2019 International Conference on Computer, Control, Informatics and its Applications (IC3INA)},
  pages={19--24},
  year={2019},
  organization={IEEE}
}

@inproceedings{DBLP:conf/naacl/DevlinCLT19,
  author    = {Jacob Devlin and
               Ming{-}Wei Chang and
               Kenton Lee and
               Kristina Toutanova},
  editor    = {Jill Burstein and
               Christy Doran and
               Thamar Solorio},
  title     = {{BERT:} Pre-training of Deep Bidirectional Transformers for Language
               Understanding},
  booktitle = {Proceedings of the 2019 Conference of the North American Chapter of
               the Association for Computational Linguistics: Human Language Technologies,
               {NAACL-HLT} 2019, Minneapolis, MN, USA, June 2-7, 2019, Volume 1 (Long
               and Short Papers)},
  pages     = {4171--4186},
  publisher = {Association for Computational Linguistics},
  year      = {2019},
  url       = {https://doi.org/10.18653/v1/n19-1423},
  doi       = {10.18653/v1/n19-1423},
  timestamp = {Fri, 06 Aug 2021 00:41:31 +0200},
  biburl    = {https://dblp.org/rec/conf/naacl/DevlinCLT19.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{DBLP:journals/corr/abs-2102-01757,
  author    = {Elizabeth Salesky and
               Matthew Wiesner and
               Jacob Bremerman and
               Roldano Cattoni and
               Matteo Negri and
               Marco Turchi and
               Douglas W. Oard and
               Matt Post},
  title     = {The Multilingual TEDx Corpus for Speech Recognition and Translation},
  journal   = {CoRR},
  volume    = {abs/2102.01757},
  year      = {2021},
  url       = {https://arxiv.org/abs/2102.01757},
  eprinttype = {arXiv},
  eprint    = {2102.01757},
  timestamp = {Tue, 09 Feb 2021 13:35:56 +0100},
  biburl    = {https://dblp.org/rec/journals/corr/abs-2102-01757.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{DBLP:journals/csl/CattoniGBNT21,
  author    = {Roldano Cattoni and
               Mattia Antonino Di Gangi and
               Luisa Bentivogli and
               Matteo Negri and
               Marco Turchi},
  title     = {MuST-C: {A} multilingual corpus for end-to-end speech translation},
  journal   = {Comput. Speech Lang.},
  volume    = {66},
  pages     = {101155},
  year      = {2021},
  url       = {https://doi.org/10.1016/j.csl.2020.101155},
  doi       = {10.1016/j.csl.2020.101155},
  timestamp = {Thu, 17 Dec 2020 16:21:15 +0100},
  biburl    = {https://dblp.org/rec/journals/csl/CattoniGBNT21.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}


@inproceedings{vaswani2017attention,
  title={Attention is all you need},
  author={Vaswani, Ashish and Shazeer, Noam and Parmar, Niki and Uszkoreit, Jakob and Jones, Llion and Gomez, Aidan N and Kaiser, {\L}ukasz and Polosukhin, Illia},
  booktitle={Advances in neural information processing systems},
  pages={5998--6008},
  year={2017}
}

@inproceedings{he2016deep,
  title={Deep residual learning for image recognition},
  author={He, Kaiming and Zhang, Xiangyu and Ren, Shaoqing and Sun, Jian},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={770--778},
  year={2016}
}


@inproceedings{DBLP:conf/nips/BaevskiZMA20,
  author    = {Alexei Baevski and
               Yuhao Zhou and
               Abdelrahman Mohamed and
               Michael Auli},
  editor    = {Hugo Larochelle and
               Marc'Aurelio Ranzato and
               Raia Hadsell and
               Maria{-}Florina Balcan and
               Hsuan{-}Tien Lin},
  title     = {wav2vec 2.0: {A} Framework for Self-Supervised Learning of Speech
               Representations},
  booktitle = {Advances in Neural Information Processing Systems 33: Annual Conference
               on Neural Information Processing Systems 2020, NeurIPS 2020, December
               6-12, 2020, virtual},
  year      = {2020},
  url       = {https://proceedings.neurips.cc/paper/2020/hash/92d1e1eb1cd6f9fba3227870bb6d7f07-Abstract.html},
  timestamp = {Tue, 19 Jan 2021 15:57:22 +0100},
  biburl    = {https://dblp.org/rec/conf/nips/BaevskiZMA20.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}


@article{DBLP:journals/corr/abs-2006-13979,
  author    = {Alexis Conneau and
               Alexei Baevski and
               Ronan Collobert and
               Abdelrahman Mohamed and
               Michael Auli},
  title     = {Unsupervised Cross-lingual Representation Learning for Speech Recognition},
  journal   = {CoRR},
  volume    = {abs/2006.13979},
  year      = {2020},
  url       = {https://arxiv.org/abs/2006.13979},
  eprinttype = {arXiv},
  eprint    = {2006.13979},
  timestamp = {Wed, 01 Jul 2020 15:21:23 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-2006-13979.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/interspeech/ZelaskoSMSCD18,
  author    = {Piotr Zelasko and
               Piotr Szymanski and
               Jan Mizgajski and
               Adrian Szymczak and
               Yishay Carmiel and
               Najim Dehak},
  editor    = {B. Yegnanarayana},
  title     = {Punctuation Prediction Model for Conversational Speech},
  booktitle = {Interspeech 2018, 19th Annual Conference of the International Speech
               Communication Association, Hyderabad, India, 2-6 September 2018},
  pages     = {2633--2637},
  publisher = {{ISCA}},
  year      = {2018},
  url       = {https://doi.org/10.21437/Interspeech.2018-1096},
  doi       = {10.21437/Interspeech.2018-1096},
  timestamp = {Sun, 25 Jul 2021 11:53:16 +0200},
  biburl    = {https://dblp.org/rec/conf/interspeech/ZelaskoSMSCD18.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/interspeech/StolckeSBOHPTL98,
  author    = {Andreas Stolcke and
               Elizabeth Shriberg and
               Rebecca A. Bates and
               Mari Ostendorf and
               Dilek Zeynep Hakkani and
               Madelaine Plauch{\'{e}} and
               G{\"{o}}khan T{\"{u}}r and
               Yu Lu},
  title     = {Automatic detection of sentence boundaries and disfluencies based
               on recognized words},
  booktitle = {The 5th International Conference on Spoken Language Processing, Incorporating
               The 7th Australian International Speech Science and Technology Conference,
               Sydney Convention Centre, Sydney, Australia, 30th November - 4th December
               1998},
  publisher = {{ISCA}},
  year      = {1998},
  url       = {http://www.isca-speech.org/archive/icslp\_1998/i98\_0059.html},
  timestamp = {Mon, 22 Jul 2019 16:11:38 +0200},
  biburl    = {https://dblp.org/rec/conf/interspeech/StolckeSBOHPTL98.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/icassp/BeefermanBL98,
  author    = {Doug Beeferman and
               Adam L. Berger and
               John D. Lafferty},
  title     = {Cyberpunc: a lightweight punctuation annotation system for speech},
  booktitle = {Proceedings of the 1998 {IEEE} International Conference on Acoustics,
               Speech and Signal Processing, {ICASSP} '98, Seattle, Washington, USA,
               May 12-15, 1998},
  pages     = {689--692},
  publisher = {{IEEE}},
  year      = {1998},
  url       = {https://doi.org/10.1109/ICASSP.1998.675358},
  doi       = {10.1109/ICASSP.1998.675358},
  timestamp = {Wed, 16 Oct 2019 14:14:52 +0200},
  biburl    = {https://dblp.org/rec/conf/icassp/BeefermanBL98.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/naacl/ShieberT03,
  author    = {Stuart M. Shieber and
               Xiaopeng Tao},
  editor    = {Marti A. Hearst and
               Mari Ostendorf},
  title     = {Comma Restoration Using Constituency Information},
  booktitle = {Human Language Technology Conference of the North American Chapter
               of the Association for Computational Linguistics, {HLT-NAACL} 2003,
               Edmonton, Canada, May 27 - June 1, 2003},
  publisher = {The Association for Computational Linguistics},
  year      = {2003},
  url       = {https://aclanthology.org/N03-1029/},
  timestamp = {Fri, 06 Aug 2021 00:41:32 +0200},
  biburl    = {https://dblp.org/rec/conf/naacl/ShieberT03.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/interspeech/HuangZ02,
  author    = {Jing Huang and
               Geoffrey Zweig},
  editor    = {John H. L. Hansen and
               Bryan L. Pellom},
  title     = {Maximum entropy model for punctuation annotation from speech},
  booktitle = {7th International Conference on Spoken Language Processing, {ICSLP2002}
               - {INTERSPEECH} 2002, Denver, Colorado, USA, September 16-20, 2002},
  publisher = {{ISCA}},
  year      = {2002},
  url       = {http://www.isca-speech.org/archive/icslp\_2002/i02\_0917.html},
  timestamp = {Thu, 20 Feb 2020 18:58:04 +0100},
  biburl    = {https://dblp.org/rec/conf/interspeech/HuangZ02.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/interspeech/UeffingBV13,
  author    = {Nicola Ueffing and
               Maximilian Bisani and
               Paul Vozila},
  editor    = {Fr{\'{e}}d{\'{e}}ric Bimbot and
               Christophe Cerisara and
               C{\'{e}}cile Fougeron and
               Guillaume Gravier and
               Lori Lamel and
               Fran{\c{c}}ois Pellegrino and
               Pascal Perrier},
  title     = {Improved models for automatic punctuation prediction for spoken and
               written text},
  booktitle = {{INTERSPEECH} 2013, 14th Annual Conference of the International Speech
               Communication Association, Lyon, France, August 25-29, 2013},
  pages     = {3097--3101},
  publisher = {{ISCA}},
  year      = {2013},
  url       = {http://www.isca-speech.org/archive/interspeech\_2013/i13\_3097.html},
  timestamp = {Mon, 27 Jan 2014 20:38:49 +0100},
  biburl    = {https://dblp.org/rec/conf/interspeech/UeffingBV13.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/interspeech/ChoKNW15,
  author    = {Eunah Cho and
               Kevin Kilgour and
               Jan Niehues and
               Alex Waibel},
  title     = {Combination of {NN} and {CRF} models for joint detection of punctuation
               and disfluencies},
  booktitle = {{INTERSPEECH} 2015, 16th Annual Conference of the International Speech
               Communication Association, Dresden, Germany, September 6-10, 2015},
  pages     = {3650--3654},
  publisher = {{ISCA}},
  year      = {2015},
  url       = {http://www.isca-speech.org/archive/interspeech\_2015/i15\_3650.html},
  timestamp = {Mon, 04 Jan 2016 19:12:52 +0100},
  biburl    = {https://dblp.org/rec/conf/interspeech/ChoKNW15.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/iwslt/PeitzFMN11,
  author    = {Stephan Peitz and
               Markus Freitag and
               Arne Mauser and
               Hermann Ney},
  title     = {Modeling punctuation prediction as machine translation},
  booktitle = {2011 International Workshop on Spoken Language Translation, {IWSLT}
               2011, San Francisco, CA, USA, December 8-9, 2011},
  pages     = {238--245},
  publisher = {{ISCA}},
  year      = {2011},
  url       = {http://www.isca-speech.org/archive/iwslt\_11/sltb\_238.html},
  timestamp = {Mon, 31 Mar 2014 16:34:17 +0200},
  biburl    = {https://dblp.org/rec/conf/iwslt/PeitzFMN11.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{lecun2015deep,
  title={Deep learning},
  author={LeCun, Yann and Bengio, Yoshua and Hinton, Geoffrey},
  journal={nature},
  volume={521},
  number={7553},
  pages={436--444},
  year={2015},
  publisher={Nature Publishing Group}
}

% @inproceedings{DBLP:conf/interspeech/TilkA15,
%   author    = {Ottokar Tilk and
%               Tanel Alum{\"{a}}e},
%   title     = {{LSTM} for punctuation restoration in speech transcripts},
%   booktitle = {{INTERSPEECH} 2015, 16th Annual Conference of the International Speech
%               Communication Association, Dresden, Germany, September 6-10, 2015},
%   pages     = {683--687},
%   publisher = {{ISCA}},
%   year      = {2015},
%   url       = {http://www.isca-speech.org/archive/interspeech\_2015/i15\_0683.html},
%   timestamp = {Mon, 04 Jan 2016 19:12:52 +0100},
%   biburl    = {https://dblp.org/rec/conf/interspeech/TilkA15.bib},
%   bibsource = {dblp computer science bibliography, https://dblp.org}
% }

@inproceedings{DBLP:conf/interspeech/TilkA16,
  author    = {Ottokar Tilk and
               Tanel Alum{\"{a}}e},
  editor    = {Nelson Morgan},
  title     = {Bidirectional Recurrent Neural Network with Attention Mechanism for
               Punctuation Restoration},
  booktitle = {Interspeech 2016, 17th Annual Conference of the International Speech
               Communication Association, San Francisco, CA, USA, September 8-12,
               2016},
  pages     = {3047--3051},
  publisher = {{ISCA}},
  year      = {2016},
  url       = {https://doi.org/10.21437/Interspeech.2016-1517},
  doi       = {10.21437/Interspeech.2016-1517},
  timestamp = {Fri, 29 Jan 2021 17:41:26 +0100},
  biburl    = {https://dblp.org/rec/conf/interspeech/TilkA16.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/hlt/Salimbajevs16,
  author    = {Askars Salimbajevs},
  editor    = {Inguna Skadina and
               Roberts Rozis},
  title     = {Bidirectional {LSTM} for Automatic Punctuation Restoration},
  booktitle = {Human Language Technologies - The Baltic Perspective - Proceedings
               of the Seventh International Conference Baltic {HLT} 2016, Riga, Latvia,
               October 6-7, 2016},
  series    = {Frontiers in Artificial Intelligence and Applications},
  volume    = {289},
  pages     = {59--65},
  publisher = {{IOS} Press},
  year      = {2016},
  url       = {https://doi.org/10.3233/978-1-61499-701-6-59},
  doi       = {10.3233/978-1-61499-701-6-59},
  timestamp = {Mon, 08 Feb 2021 13:26:33 +0100},
  biburl    = {https://dblp.org/rec/conf/hlt/Salimbajevs16.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/slsp/TundikTS17,
  author    = {M{\'{a}}t{\'{e}} {\'{A}}kos T{\"{u}}ndik and
               Bal{\'{a}}zs Tarj{\'{a}}n and
               Gy{\"{o}}rgy Szasz{\'{a}}k},
  editor    = {Nathalie Camelin and
               Yannick Est{\`{e}}ve and
               Carlos Mart{\'{\i}}n{-}Vide},
  title     = {Low Latency MaxEnt- and RNN-Based Word Sequence Models for Punctuation
               Restoration of Closed Caption Data},
  booktitle = {Statistical Language and Speech Processing - 5th International Conference,
               {SLSP} 2017, Le Mans, France, October 23-25, 2017, Proceedings},
  series    = {Lecture Notes in Computer Science},
  volume    = {10583},
  pages     = {155--166},
  publisher = {Springer},
  year      = {2017},
  url       = {https://doi.org/10.1007/978-3-319-68456-7\_13},
  doi       = {10.1007/978-3-319-68456-7\_13},
  timestamp = {Sat, 19 Oct 2019 20:37:21 +0200},
  biburl    = {https://dblp.org/rec/conf/slsp/TundikTS17.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/bionlp/SalloumFEMS17,
  author    = {Wael Salloum and
               Greg Finley and
               Erik Edwards and
               Mark Miller and
               David Suendermann{-}Oeft},
  editor    = {Kevin Bretonnel Cohen and
               Dina Demner{-}Fushman and
               Sophia Ananiadou and
               Junichi Tsujii},
  title     = {Deep Learning for Punctuation Restoration in Medical Reports},
  booktitle = {BioNLP 2017, Vancouver, Canada, August 4, 2017},
  pages     = {159--164},
  publisher = {Association for Computational Linguistics},
  year      = {2017},
  url       = {https://doi.org/10.18653/v1/W17-2319},
  doi       = {10.18653/v1/W17-2319},
  timestamp = {Fri, 06 Aug 2021 00:41:21 +0200},
  biburl    = {https://dblp.org/rec/conf/bionlp/SalloumFEMS17.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/icpr/WangCYX18,
  author    = {Feng Wang and
               Wei Chen and
               Zhen Yang and
               Bo Xu},
  title     = {Self-Attention Based Network for Punctuation Restoration},
  booktitle = {24th International Conference on Pattern Recognition, {ICPR} 2018,
               Beijing, China, August 20-24, 2018},
  pages     = {2803--2808},
  publisher = {{IEEE} Computer Society},
  year      = {2018},
  url       = {https://doi.org/10.1109/ICPR.2018.8545470},
  doi       = {10.1109/ICPR.2018.8545470},
  timestamp = {Mon, 02 Dec 2019 19:00:56 +0100},
  biburl    = {https://dblp.org/rec/conf/icpr/WangCYX18.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/icassp/Kim19,
  author    = {Seokhwan Kim},
  title     = {Deep Recurrent Neural Networks with Layer-wise Multi-head Attentions
               for Punctuation Restoration},
  booktitle = {{IEEE} International Conference on Acoustics, Speech and Signal Processing,
               {ICASSP} 2019, Brighton, United Kingdom, May 12-17, 2019},
  pages     = {7280--7284},
  publisher = {{IEEE}},
  year      = {2019},
  url       = {https://doi.org/10.1109/ICASSP.2019.8682418},
  doi       = {10.1109/ICASSP.2019.8682418},
  timestamp = {Wed, 16 Oct 2019 14:14:52 +0200},
  biburl    = {https://dblp.org/rec/conf/icassp/Kim19.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{DBLP:journals/corr/abs-2004-00248,
  author    = {Jiangyan Yi and
               Jianhua Tao and
               Ye Bai and
               Zhengkun Tian and
               Cunhang Fan},
  title     = {Adversarial Transfer Learning for Punctuation Restoration},
  journal   = {CoRR},
  volume    = {abs/2004.00248},
  year      = {2020},
  url       = {https://arxiv.org/abs/2004.00248},
  eprinttype = {arXiv},
  eprint    = {2004.00248},
  timestamp = {Wed, 08 Apr 2020 17:08:25 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-2004-00248.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{DBLP:journals/corr/abs-2101-07343,
  author    = {Attila Nagy and
               Bence Bial and
               Judit {\'{A}}cs},
  title     = {Automatic punctuation restoration with {BERT} models},
  journal   = {CoRR},
  volume    = {abs/2101.07343},
  year      = {2021},
  url       = {https://arxiv.org/abs/2101.07343},
  eprinttype = {arXiv},
  eprint    = {2101.07343},
  timestamp = {Fri, 22 Jan 2021 15:16:00 +0100},
  biburl    = {https://dblp.org/rec/journals/corr/abs-2101-07343.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/iwslt/CourtlandFM20,
  author    = {Maury Courtland and
               Adam Faulkner and
               Gayle McElvain},
  editor    = {Marcello Federico and
               Alex Waibel and
               Kevin Knight and
               Satoshi Nakamura and
               Hermann Ney and
               Jan Niehues and
               Sebastian St{\"{u}}ker and
               Dekai Wu and
               Joseph Mariani and
               Fran{\c{c}}ois Yvon},
  title     = {Efficient Automatic Punctuation Restoration Using Bidirectional Transformers
               with Robust Inference},
  booktitle = {Proceedings of the 17th International Conference on Spoken Language
               Translation, {IWSLT} 2020, Online, July 9 - 10, 2020},
  pages     = {272--279},
  publisher = {Association for Computational Linguistics},
  year      = {2020},
  url       = {https://doi.org/10.18653/v1/2020.iwslt-1.33},
  doi       = {10.18653/v1/2020.iwslt-1.33},
  timestamp = {Fri, 06 Aug 2021 00:40:09 +0200},
  biburl    = {https://dblp.org/rec/conf/iwslt/CourtlandFM20.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/aclnut/AlamKA20,
  author    = {Tanvirul Alam and
               Akib Khan and
               Firoj Alam},
  editor    = {Wei Xu and
               Alan Ritter and
               Tim Baldwin and
               Afshin Rahimi},
  title     = {Punctuation Restoration using Transformer Models for High-and Low-Resource
               Languages},
  booktitle = {Proceedings of the Sixth Workshop on Noisy User-generated Text, W-NUT@EMNLP
               2020 Online, November 19, 2020},
  pages     = {132--142},
  publisher = {Association for Computational Linguistics},
  year      = {2020},
  url       = {https://doi.org/10.18653/v1/2020.wnut-1.18},
  doi       = {10.18653/v1/2020.wnut-1.18},
  timestamp = {Fri, 06 Aug 2021 00:40:09 +0200},
  biburl    = {https://dblp.org/rec/conf/aclnut/AlamKA20.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/interspeech/YiTTBF20,
  author    = {Jiangyan Yi and
               Jianhua Tao and
               Zhengkun Tian and
               Ye Bai and
               Cunhang Fan},
  editor    = {Helen Meng and
               Bo Xu and
               Thomas Fang Zheng},
  title     = {Focal Loss for Punctuation Prediction},
  booktitle = {Interspeech 2020, 21st Annual Conference of the International Speech
               Communication Association, Virtual Event, Shanghai, China, 25-29 October
               2020},
  pages     = {721--725},
  publisher = {{ISCA}},
  year      = {2020},
  url       = {https://doi.org/10.21437/Interspeech.2020-1638},
  doi       = {10.21437/Interspeech.2020-1638},
  timestamp = {Fri, 29 Jan 2021 17:40:17 +0100},
  biburl    = {https://dblp.org/rec/conf/interspeech/YiTTBF20.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/icassp/HentschelTO21,
  author    = {Michael Hentschel and
               Emiru Tsunoo and
               Takao Okuda},
  title     = {Making Punctuation Restoration Robust and Fast with Multi-Task Learning
               and Knowledge Distillation},
  booktitle = {{IEEE} International Conference on Acoustics, Speech and Signal Processing,
               {ICASSP} 2021, Toronto, ON, Canada, June 6-11, 2021},
  pages     = {7773--7777},
  publisher = {{IEEE}},
  year      = {2021},
  url       = {https://doi.org/10.1109/ICASSP39728.2021.9414518},
  doi       = {10.1109/ICASSP39728.2021.9414518},
  timestamp = {Fri, 09 Jul 2021 13:04:25 +0200},
  biburl    = {https://dblp.org/rec/conf/icassp/HentschelTO21.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{DBLP:journals/corr/abs-2107-09099,
  author    = {Qiushi Huang and
               Tom Ko and
               H. Lilian Tang and
               Xubo Liu and
               Bo Wu},
  title     = {Token-Level Supervised Contrastive Learning for Punctuation Restoration},
  journal   = {CoRR},
  volume    = {abs/2107.09099},
  year      = {2021},
  url       = {https://arxiv.org/abs/2107.09099},
  eprinttype = {arXiv},
  eprint    = {2107.09099},
  timestamp = {Thu, 29 Jul 2021 12:42:39 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-2107-09099.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/eacl/Chordia21,
  author    = {Varnith Chordia},
  editor    = {Dimitra Gkatzia and
               Djam{\'{e}} Seddah},
  title     = {PunKtuator: {A} Multilingual Punctuation Restoration System for Spoken
               and Written Text},
  booktitle = {Proceedings of the 16th Conference of the European Chapter of the
               Association for Computational Linguistics: System Demonstrations,
               {EACL} 2021, Online, April 19-23, 2021},
  pages     = {312--320},
  publisher = {Association for Computational Linguistics},
  year      = {2021},
  url       = {https://aclanthology.org/2021.eacl-demos.37/},
  timestamp = {Fri, 06 Aug 2021 00:40:45 +0200},
  biburl    = {https://dblp.org/rec/conf/eacl/Chordia21.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/interspeech/LiL20b,
  author    = {Xinxing Li and
               Edward Lin},
  editor    = {Helen Meng and
               Bo Xu and
               Thomas Fang Zheng},
  title     = {A 43 Language Multilingual Punctuation Prediction Neural Network Model},
  booktitle = {Interspeech 2020, 21st Annual Conference of the International Speech
               Communication Association, Virtual Event, Shanghai, China, 25-29 October
               2020},
  pages     = {1067--1071},
  publisher = {{ISCA}},
  year      = {2020},
  url       = {https://doi.org/10.21437/Interspeech.2020-2052},
  doi       = {10.21437/Interspeech.2020-2052},
  timestamp = {Fri, 29 Jan 2021 17:41:29 +0100},
  biburl    = {https://dblp.org/rec/conf/interspeech/LiL20b.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/interspeech/TundikSGB18,
  author    = {M{\'{a}}t{\'{e}} {\'{A}}kos T{\"{u}}ndik and
               Gy{\"{o}}rgy Szasz{\'{a}}k and
               G{\'{a}}bor Gosztolya and
               Andr{\'{a}}s Beke},
  editor    = {B. Yegnanarayana},
  title     = {User-centric Evaluation of Automatic Punctuation in {ASR} Closed Captioning},
  booktitle = {Interspeech 2018, 19th Annual Conference of the International Speech
               Communication Association, Hyderabad, India, 2-6 September 2018},
  pages     = {2628--2632},
  publisher = {{ISCA}},
  year      = {2018},
  url       = {https://doi.org/10.21437/Interspeech.2018-1352},
  doi       = {10.21437/Interspeech.2018-1352},
  timestamp = {Fri, 21 May 2021 08:16:43 +0200},
  biburl    = {https://dblp.org/rec/conf/interspeech/TundikSGB18.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{vandeghinste2018comparison,
  title={A comparison of different punctuation prediction approaches in a translation context},
  author={Vandeghinste, Vincent and Verwimp, Lyan and Pelemans, Joris and Wambacq, Patrick},
  booktitle={Proceedings of the 21st Annual Conference of the European Association for Machine Translation: 28-30 May 2018, Universitat d'Alacant, Alacant, Spain},
  pages={269--278},
  year={2018},
  organization={European Association for Machine Translation}
}

@inproceedings{cureg2019sentiment,
  title={Sentiment analysis on tweets with punctuations, emoticons, and negations},
  author={Cureg, Miks Q and De La Cruz, Juan Aurel D and Solomon, Juan Carlos A and Saharkhiz, Aresh T and Balan, Ariel Kelly D and Samonte, Mary Jane C},
  booktitle={Proceedings of the 2019 2nd International Conference on Information Science and Systems},
  pages={266--270},
  year={2019}
}

@inproceedings{DBLP:conf/interspeech/MakhoulBBNRSSX05,
  author    = {John Makhoul and
               Alex Baron and
               Ivan Bulyko and
               Long Nguyen and
               Lance A. Ramshaw and
               David Stallard and
               Richard M. Schwartz and
               Bing Xiang},
  title     = {The effects of speech recognition and punctuation on information extraction
               performance},
  booktitle = {{INTERSPEECH} 2005 - Eurospeech, 9th European Conference on Speech
               Communication and Technology, Lisbon, Portugal, September 4-8, 2005},
  pages     = {57--60},
  publisher = {{ISCA}},
  year      = {2005},
  url       = {http://www.isca-speech.org/archive/interspeech\_2005/i05\_0057.html},
  timestamp = {Sun, 13 Mar 2011 19:32:30 +0100},
  biburl    = {https://dblp.org/rec/conf/interspeech/MakhoulBBNRSSX05.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

==> tables/2-f1-score-audio-dataset.tex <==
\begin{table}[h]
\centering
\footnotesize	
\caption{F1 score for three punctuations and overall micro-F1 on English-Audio test set.}
\label{Tab:results-on-english-audio}
\begin{tabular}{l|cccc}
\hline
             & Overall   & Comma & Full Stop   & Question Mark   \\ \hline
Self-Att Vec & @zym      &       &      &      \\
BERT         & 77.4      & 70.8  & 81.2 & 79.5 \\ 
MuSe         & 77.9      & 73.2  & 83.6 & 79.4 \\ 
MuSe  + TTS       & @zym      &   &  &  \\ 
\hline
MMBP-Audio         & 78.5      & 74.2  & 84.3 & 80.8 \\ 
MMBP-Mix     & @zym      &       &      &      \\ \hline
\end{tabular}
\end{table}

==> tables/3-f1-score-mix-dataset.tex <==
\begin{table}[h]
\centering
\caption{F1 score for three punctuations and overall micro-F1 on Multi-Mix Dataset.}
\label{Tab:results-on-multi-mix}
\footnotesize
\begin{tabular}{l|cccc}
\hline
             & Overall   & Comma & Full Stop   & Question Mark   \\ \hline
Att-GRU          & @wlw &       &      &      \\
BLSTM-T    & @wlw      &       &      &      \\
BERT         & TODO      &  &  &  \\ \hline
\method-Mix         & @zym      &      &    &    \\ \hline
\end{tabular}


\end{table}
